REVEAL: Retrieval-Augmented Visual-Language Pre-Training with Multi-Source Multimodal Knowledge Memory

In this paper, we propose an end-to-end Retrieval-Augmented Visual Language Model (REVEAL) that learns to encode world knowledge into a large-scale memory, and to retrieve from it to answer knowledge-intensive queries. REVEAL consists of four key components: the memory, the encoder, the retriever and the generator. The large-scale memory encodes various sources of multimodal world knowledge (e.g. image-text pairs, question answering pairs, knowledge graph triplets, etc) via a unified encoder. The retriever finds the most relevant knowledge entries in the memory, and the generator fuses the retrieved knowledge with the input query to produce the output. A key novelty in our approach is that the memory, encoder, retriever and generator are all pre-trained end-to-end on a massive amount of data. Furthermore, our approach can use a diverse set of multimodal knowledge sources, which is shown to result in significant gains. We show that REVEAL achieves state-of-the-art results on visual question answering and image captioning.

==> sections/old_approach_nov7.tex <==
\begin{figure*}[t!]
    \hspace{-.1in}
    \centering
    \includegraphics[width=2.1\columnwidth]{figures/memory_framework.png}
    \caption{\textbf{Overall workflow of \method} could be splitted into four steps: a) Input Query Encoding, which encodes a multi-modal input (text-only, image-only or image-text pair) into a sequence of token embeddings, followed by a query head to also get a single query embedding; and b) retrieved Top-K relevant knowledge entries by using the query embedding to first select corpus and next sort knowledge entries from it via Maximum-Inner-Product-Search (MIPS) over all pre-indexed key embeddings. Afterwards it c) returns either the pre-computed stale value embeddings or re-encoding the raw knowledge data to get up-to-date value embeddings as retrieved top-K knowledge. \cordelia{what do you mean by stale? when would be recompute?}
    Finally d) we fuse the retrieved top-k knowledge into a fusion layer. We inject retrieval score as prior every time we calculate attention score so that the retriever could be learned through end-to-end generative pre-training, to rank important knowledge entries higher. \cordelia{please describe e, use in the illustration the corpora we use in the paper} }
    \label{fig:framework}
    \vspace{-.1in}
\end{figure*}



\cordelia{strucutre of the method section;
I would have an overview section which includes the preliminary and challenge and clear describe the different modules in figure 1; then have a section per module; }

\cordelia{figure 1: much improved; the memory part takes a lot of space and is not described in the caption}

In this section, we first formalize the retrieval-augmented generative pre-training process in Sec.~\ref{sec:preliminary} and introduce unique challenges in multimodal setup. We then introduce the model architecture of our proposed Multimodal-Retrieval-Augmented Visual Language Model (\method) in Sec.~\ref{sec:architecture}, and how we conduct end-to-end pre-training on large-scale image-text datasets in Sec.~\ref{sec:training}. Figure~\ref{fig:framework} illustrates the overall workflow of \method.


% \paragraph{Overview of \method}
% We illustrate the overall architecture of \method in Figure~\ref{fig:framework}. The key component of \method is the Unified Multi-Modal Knowledge Memory (\memory), which stores each knowledge entry $z$ from different corpus in the form of key and value embeddings. The key is a single embedding and value is a sequence of embeddings. This layer provides an interface to enable Vision-Language model to interact with outside knowledge corpus in a differentiable manner.


% The whole forward procedure could be splitted into four steps: a) Input Encoding, which encodes a multi-modal input (text-only, image-only or image-text pair) into a sequence of token embeddings, followed by a query head to also get a single embedding; and b) Top-K Online Retrieval, which uses the query embedding to conduct dense maximum-inner-product-search (MIPS) over all key embeddings stored in \memory. We also have a gating layer to decide which knowledge corpus is more important to this query; after it c) return stale or re-encoded value, which either returning the value embeddings stored in \memory or retrieve raw data inputs to re-encode and get up-to-date embeddings as retrieved top-K knowledge; and d) Re-Rank then Decode, which passes the input embeddings with the retrieved knowledges into a fusion-in re-ranker to further decide which knowledge is more useful for this task, and the final fused embeddings are passed to decoder for generation. We also multiply the pairwise retrieval score into the fusion layer so that it could receive similar gradients as re-ranking for gradually improve the retrieval quality through generative pre-training. 

\subsection{Preliminary: Retrieval-Generation Pipeline} \label{sec:preliminary}

Our method follows the retrieval-augmented generation approach~\cite{DBLP:conf/nips/LewisPPPKGKLYR020,DBLP:journals/corr/abs-2007-01282} which allows neural generator to access and retrieve relevant evidence from outside knowledge source, so that model do not needs to memorize all required knowledge. One key difference of this paper compared with previous ones is that we aim to utilize a diverse set of multi-modal knowledge corpora (e.g., WikiData knowledge graph, Wikimedia image-text pairs, etc). We denote each corpus as $\mathcal{C}^i = \{z^i_1, \dots, z^i_M\}$, in which each $z^i_j \in \mathcal{C}^i$ could be an image-text pair, text only, image only, or triplets from knowledge graph, etc.
% \alireza{could be an image-text pair, text only, image only, or triplets from knowledge graph, etc.}.
We denote the unified knowledge corpus $\mathcal{C} = \mathcal{C}^1 \cup \mathcal{C}^2 \dots \cup \mathcal{C}^N$ combing $N$ different knowledge corpora. 


For both pre-training and fine-tuning, the goal of \method model is to learn a distribution $P(y \mid x)$ to generate textual output $y$ given multi-modal input query $x$. 
To incorporate outside knowledge into this generation process, we include a latent variable $\mathcal{Z}$ denoted as a set of $K$ knowledge $\mathcal{Z} = \{z_1, \dots, z_K\} \subset \mathcal{C}$ relevant to query $x$. Note that in our setup, each $z$ could be retrieved from diverse knowledge sources with different modality.
\method is thus a latent variable model 
\alireza{what does it mean to be a latent variable model?}
consisting of two components: (1) a \textbf{neural retriever} with parameter $\theta$ retrieves relevant Top-K knowledge set $\mathcal{Z}$ from unified knowledge corpus $\mathcal{C}$, which could be formalized as $p(\mathcal{Z} \mid x; \mathcal{C}, \theta)$ 
% \alireza{I think it is $p(\mathcal{Z} \mid x,\mathcal{C}; \theta)$} 
and (2) a \textbf{neural generator} with parameter $\rho$ conditioned on both input $x$ and retrieved knowledge $\mathcal{Z}$ to model $p(y \mid x, \mathcal{Z}; \rho)$ 
With such two steps, we then could decompose $p(y \mid x; \theta, \rho, \mathcal{C})$ as:
\begin{align}
    p(y  \mid  x; \theta, \rho, \mathcal{C}) = \sum_{\mathcal{Z} \subset \mathcal{C}}  \underbrace{p(\mathcal{Z}  \mid  x; \theta, \mathcal{C})}_{retrieval} \cdot  \underbrace{p(y  \mid  \mathcal{Z}, x; \rho)}_{generation} \label{eq:main} 
\end{align}
% \alireza{Not sure why there is a $\Sigma$ in the above formula.}
The training objective is to find $\theta$ and $\rho$ to maximize the overall likelihood. 

\paragraph{Challenges for Multimodal-Retrieval Training}

Many previous works in both NLP and CV domains have tried to augment model with an outside knowledge source. However, most of these works are focusing on a single domain, in which $x$ and $z$ are of the same modality. Therefore, a naive solution is to train a good neural representation model in particular domain, and then simply fix it to be the retriever~\cite{DBLP:conf/icml/ChenK0H20,DBLP:journals/corr/abs-2004-04906} to augment downstream models.

However, as we discuss in the introduction, for those tasks that require diverse knowledge with different modalities, by far there is no a single unified pre-trained off-the-shelf model that could encode data from arbitrary modality into same space for retrieval. In addition, to train dedicated multimodal retrieval, it is arguous or even impossible to collect supervised retrieval ground-truth across different modalities.

Therefore, following the recent trend that learning foundation model over unlabelled corpus, we seek to also train the multimodal retriever $p(\mathcal{Z}  \mid  x; \theta, \mathcal{C})$ directly from the generative pre-training. Most existing works that jointly train retriever with generator in NLP domains concatenate each retrieved knowledge $z$ with input $x$ independently without considering the mutual dependency of these retrieved knowledge, and use the corresponding generative loss to evaluate how important each knowledge $z$ is to the task. However, for multimodal setup there exist some unique challenges. Firstly it's impossible to simply fuse $z$ of different modality with $x$ at raw input space, but we need to map them to the same latent space. Secondly as we are aiming the problems that require multiple knowledge (e.g., up to 100 from different sources), they are definitely not mutually independent. One typical example is the multi-hop question answering~\cite{DBLP:conf/emnlp/Yang0ZBCSM18} that require a chain of reasoning path to reach final answer, in which case the retrieved knowledge has sequential dependency and could not be evaluated separately. Therefore, how to jointly estimate the importance of each knowledge with different modality is the key challenge that our \method aims to solve. We will introduce how we conduct efficient joint pre-training of both retriever and generator in the following.




% Directly optimizing Eq.\ref{eq:main} is intractable as it needs to summing over all combination of top-K knowledge from corpus $\mathcal{Z}$. As an alternative, many previous work following~\cite{DBLP:journals/corr/abs-2002-08909, DBLP:conf/nips/SachanRHDY21F} resort to instead optimize the estimated posterior of $z$. Specifically, $p(z | q, y) \propto p(y | q, z) \cdot p(z | q)$, which means they could utilize $p(y | q, z)$, meaning how retrieved documents help generate 






\subsection{Model Architecture of \method} \label{sec:architecture}

\alireza{I am not sure if we want a sub-section here. It could be continuation of 3.1 here.}
\method consists of two key components, 1) multi-modal knowledge retrieval, which models $p(\mathcal{Z}  \mid x; \theta, \mathcal{C})$, and 2) attentive knowledge fusion and decoding, which models $p(y  \mid \mathcal{Z},x ; \rho)$.

\paragraph{Retrieving from Multi-Modal Knowledge Sources}
Given input query $x$, knowledge retriever aims to find a set of knowledge $\mathcal{Z} = \{z^j_i\}$ with highest probability to contain evidence helpful for this task. As directly modelling probability of set over large space is very hard, we approximate it by assuming that we retrieve each knowledge entry independently,
\alireza{This is not described well. I guess you want to say every retrieved example is used independently for reasoning?}
such that $p(\mathcal{Z} \mid x ; \theta, \mathcal{C}) = \prod_{z^j_i \in \mathcal{Z}} p(z^j_i \mid x ; \theta, \mathcal{C})$. We thus could simply select knowledge with Top-K $p(z^j_i \mid x ; \theta, \mathcal{C})$ score.


% \alireza{Is previous work REALM? are there more works that you are refering to here? Mabye instead of calling them previous work cite them here.} 

Note that we consider retrieving from multiple knowledge sources, where each represent different aspects of world knowledge. To accomplish it, we model the retrieval score $p(z^j_i \mid x ; \theta, \mathcal{C})$ in two steps: firstly select which knowledge corpus $\mathcal{C}^j$ to use based on the query $x$ via a learnable corpus gating, and next find knowledge within corresponding corpus that are relevant to this query. More specifically:
% finding top-K relevant knowledge set $\mathcal{Z} = \{z^j_i\}$ from knowledge corpus $\mathcal{C}^j$ that might contain evidence for query $x$. As   We adopt dual-encoder architecture with an additional corpus selection gate to model $p(z^j_i \mid x ; \theta)$: 
% After retrieving the top-K results independently, we use a Transformer-based Re-Ranker to estimate more accurate retrieval results. In the following we introduce the first independent retrieval step:
\begin{align}
    & p(z^j_i \mid x ; \theta, \mathcal{C})  =  p(\mathcal{C}^j \mid x ; \theta, \mathcal{C}) \cdot p(z^j_i \mid x ; \theta, \mathcal{C}^j) \\
    &= Gate_{\mathcal{C}^j}(x) \cdot \frac{\exp\big( Rel(x, z^j_i) / \tau \big) }{\sum_{z^{j}_{k} \in \mathcal{C}^j} \exp\big( Rel(x, z^{j}_{k}) / \tau \big)}   \label{eq:retrieve}
\end{align}
where $Gate_{\mathcal{C}^j}(x)=\text{Softmax}(W\cdot \texttt{Embed}_Q(x) + b)[j]$ is a Softmax gating modelling
which knowledge corpus to retrieve from given each query, i.e., $p(\mathcal{C}^j \mid x ; \theta, \mathcal{C})$, and
$Rel(x,z^j_i)$ denotes relevance score between query $x$ and each knowledge entry $z^j_i \in \mathcal{C}^j$. We implement relevance score via a bi-encoder architecture~\cite{DBLP:conf/nips/BromleyGLSS93}, such that $Rel(x,z^j_i) = \texttt{Embed}_Q(x)^T \cdot \texttt{Embed}_K(z^j_i)$ is the inner product of $d$-dimensional query and key embeddings.


%     & Gate(x, \mathcal{C}^j) = \frac{\exp \big( W^{\mathcal{C}}_j \cdot \texttt{Embed}_Q(x) + b^{\mathcal{C}}_j \big)}{ \sum_{k} \exp \big( W^{\mathcal{C}}_k \cdot \texttt{Embed}_Q(x) + b^{\mathcal{C}}_k \big)}, \\
%     & Rel(x,z^j_i) = \texttt{Embed}_Q(x)^T \cdot \texttt{Embed}_K(z^j_i). 
% \end{align}



To model multiple modalities via a single model, we firstly use a unified base V-L Encoder $f(\cdot)$ encode multi-modal input (in the format of text-only, image-only or image-text pair) for both query $x$ or knowledge $z$ into sequence of embeddings.
We adopt a Vision Transformer (ViT) and lower-layer T5 Encoder to encode image and text separately, and then add a projection layer over ViT to map image tokens into the same space of text tokens. We eventually concatenate the two modalities as $f(x) \in \mathbb{R}^{\#token \times d}$, where $\#token$ is the number of text tokens plus number of patches for ViT. We use pre-trained ViT checkpoints trained via image-text matching~\cite{DBLP:conf/cvpr/Zhai0HB22} and pre-trained T5 checkpoint as initialization. 
% For some large ViT encoders, we froze the lower layers to save on-device memories.
On top of the encoded tokens, we use multi-layer Transformer as Query Head $\phi_Q(\cdot)$ and Key Head $\phi_K(\cdot)$, and take the output of the first \texttt{[CLS]} token to summarize the whole input data: $\texttt{Embed}_{\{Q/K\}}(x) = \phi_{\{Q/K\}}\big(f(x)\big)\texttt{[CLS]}$.
Both $\phi_K(\cdot)$ and $\phi_Q(\cdot)$ are initialized via upper-layer T5 Encoder followed by a linear projection and L2 normalization. 
% We discuss the initialization end-to-end training framework details in Sec.~\ref{sec:train}.


\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/fusion.png}
    \caption{Detailed procedure of attentive knowledge fusion module. We inject retrieval probability as a prior to knowledge token embeddings, so that the retriever could receive gradients via back-propagating over \{self/cross\}-attention part.}
    \label{fig:fusion}
\end{figure}



\paragraph{Attentive Knowledge Fusion \& Decoding}

Given the retrieved Top-K knowledge set $\mathcal{Z}=\{z_i\}_{i=1}^K$. We then introduce how we fuse the retrieved knowledge into neural generator to model $p(y \mid \mathcal{Z}, x; \rho)$.

A natural solution in NLP domain of fusing multiple knowledge would be concatenating all textual tokens and feed into Transformer-based Encoder-Decoder pipeline~\cite{DBLP:conf/nips/LewisPPPKGKLYR020}. This require quadratic complexity to the total number of tokens for self attention in Encoder part. To reduce computation,
one of the recent State-of-the-art question answering models, the Fusion-in-Decoder (FiD)~\cite{DBLP:journals/corr/abs-2007-01282} model, propose to independently encode each knowledge and concatenate them at the end until passing to decoder.
They show that by increasing the number of retrieved knowledge, the performance keeps improving when retrieving up to hundreds of knowledge. 

% A natural solution in NLP domain of fusing multiple knowledge would be concatenating all textual tokens and feed into Transformer-based Encoder-Decoder pipeline~\cite{DBLP:conf/nips/LewisPPPKGKLYR020}. This require quadratic complexity to the total number of tokens for self attention in Encoder part. To reduce computation, another widely used architecture Fusion-in-Decoder (FiD)~\cite{DBLP:journals/corr/abs-2007-01282} concatenate each knowledge with the short question, independently encode them to be a sequence of token embeddings, concatenate them and feed into decoder. 
% However, image data cannot be concatenated at raw pixel space, and could only be fused at intermediate latent space. In addition, the token length for image query are always much longer than short questions. 


For the multimodal setup that we aim to solve, we also expect to retrieve up-to-hundred knowledges, but wish to fuse them together for joint reasoning instead of encoding each independently. We thus propose an alternative way for efficient fusion. Instead of reducing the attention window as FiD, we propose to compress the original full sequence of knowledge tokens into a much shorter sequence. To accomplish this goal, we utilize the Perceiver architecture~\cite{DBLP:conf/icml/JaegleGBVZC21}, which utilizes standard Transformer-like decoder taking a $c$-length $d$-dimentional latent embedding sequence as query, and the full token sequence (i.e., the image-text pairs as retrieved knowledge) to be compressed as key and value. In this way, Perceiver $\psi(\cdot)$ could compresses the multi-modal knowledge to be arbitrary length defined by the latent query, such that $\psi(f(z)) \in \mathbb{R}^{c \times d}$ (e.g., $c=16/32$). 


To make Perceiver more suitable for knowledge compression in our \method framework, we add two additional regularization. The first is a disentangled regularization~\cite{DBLP:journals/corr/abs-2205-09797} that force every two output tokens to be linearly de-correlated $\mathcal{L}_{decor}=\sum_{i,j=1}^K \Big\lVert Covariance\big(\psi\big(f(z_i)\big), \psi\big(f(z_j)\big)\big)   \Big\rVert_F^2$, and
the other is an alignment regularization  that minimizes the L2-norm distance between the query and compressed knowledge embedding: $\mathcal{L}_{align} = \bigg \lvert 1 -  \frac{\sum_{z} \lVert \psi\big(f(z) \big) \rVert_2}{\sum_{x} \lVert f(x) \rVert_2}  \bigg \rvert$.

With the compressed tokens we then could easily concatenate all $K$ compressed knowledge embeddings with query embeddings, s.t. $E = [f(x), \psi(f(z_1)), \dots, , \psi(f(z_K))] \in \mathbb{R}^{(I + c \cdot K) \times d}$, where $I$ is the number of tokens for input query $x$. We then feed $E$ as input to a multi-layer Transformer fusion layer $F(\cdot)$. This component could learns the interaction between all these knowledge and question via self-attention to identify most important information. 
We could then passed the fused representation $F(E)$ to T5 decoder $g$ to generate output answer as $p(y | x, \mathcal{Z} ; \rho) = \prod_{t=1}^T p(y_t | y_{<t}, x, \mathcal{Z}; \rho)$, where $T$ is the number of output tokens.

\subsection{Efficient End-to-End joint training of retriever and generator} \label{sec:training}

In contrast to many previous works that train the retriever $\theta$ and generator $\rho$ separately, our method aims to learn both components jointly in an end-to-end and differentiable manner. In this following, we introduce how we modify the fusion layer to support joint training of retriever and generator via only generation loss, and also some implementation details.

\cordelia{please also mention the pretraining}
\cordelia{I don't see implementation detail\methods}


\paragraph{Retrieval as Prior to support End-to-End Training} \label{sec:train}

The training objective is to find optimal parameter $\theta$ and $\rho$ to maximize the likelihood $p(y \mid x; \theta, \rho) = \sum_{Z=\mathcal{Z}}  p(\mathcal{Z}  \mid  x; \theta) \cdot  p(y  \mid  \mathcal{Z}, x; \rho)$. The challenge is that this marginal probability involves a summation of all combination of intractable latent set variable $\mathcal{Z}$. 
One widely adopted solution is to utilize Expectation-Maximization (EM) algorithm. In the E-step we could use current-step bi-encoder retrieval model with parameter $\theta$ to find knowledge set $\mathcal{Z}_{Retr}$ with Top-K retrieval score. And in the M-step we could use it to update generator by optimizing $p(y \mid \mathcal{Z}, x; \rho)$. The problem in this way is that retriever ($\theta$) is not involved in the final answer generation procedure, and will not receive gradient to be updated in M-step. Many previous works~\cite{DBLP:journals/corr/abs-2002-08909,DBLP:conf/nips/LewisPPPKGKLYR020,DBLP:conf/nips/SachanRHDY21F} utilize alternative training signals for updating retriever, i.e., conduct generation using only each knowledge instead of all Top-K, and use corresponding generation accuracy as training signal. These ad-hoc methods are not guaranteed to be optimal for multi-knowledge retrieval, and also very inefficient if we want to retrieve up-to-hundred knowledge.

Our goal is to conduct joint end-to-end training of both retriever and generator using generation loss as guidance, without additional distant supervision step. Our solution is to inject the retrieval score as prior into the fusion and decoding process, so that retrieval model ($\theta$) could also be updated when optimizing the generative likelihood $p(y \mid \mathcal{Z}, x; \rho, \theta)$.
The detailed procedure is illustrated in Figure~\ref{fig:fusion}. At each Transformer Layer before attention calculation, we multiply the retrieval probability $p(z_i|x)$ to each token embedding belonging to knowledge $z_i$. Therefore, the attention score each knowledge send to other position $a_{:,i}$ is proportional to $p(z_i|x)$. This reflects the importance of this knowledge $z_i$ to make final prediction. By multiplying retrieval score as prior and through end-to-end training, the retriever could be learned to identify those samples that are more important to final output generation. This is similar to adopt a posterior estimation $p(z|x,y)$, which takes output answer $y$ as condition, to better optimize the retriever model. 

This modified retrieval injected fusion layer is also similar to the Mixture-of-Expert (MOE) model, in which the retrieval is like a gating layer to select knowledge, and the knowledge representation serves as the expert. In this way, we turn the discrete knowledge retrieval/selection learning into a continuous learning problem, and the whole model could be learned end-to-end.

% With this modification, in the M-step, we could simultaneously train both retriever $\theta$ and generator $\rho$, via optimizing the likelihood: $p(y | x, \mathcal{Z}_{retr}; \theta, \rho)$, given the retrieved top-K results $\mathcal{Z}_{retr}$.






% The main difference of our approach compared with EMDR$^2$ is that we don't rely on a separate decoding step to estimate posterior, instead we utilize the attention score induced by fusion-in ReRanker to serve the purpose. We introduce the details as follow.


% In the E-step, it's easy to use current bi-encoder retrieval model with parameter $\theta$ to find top-K knowledge set $\mathcal{Z}_{retr} = \arg \max_{z_1, \dots, z_K} p(z=z_i \mid x; \theta)$ by prior distribution. The challenging part is at M-step, standard model in NLP treats retrieved knowledge as input tokens, and the gradient calculated over generation $\rho$ could not be passed to retrieval parameter $\theta$. To alleviate this problem and support end-to-end differentiable training, we modify our fusion-in reranker module to inject the retrieved results earlier into attention calculation mechanism. Speficially, at each 





% This retrieval set could be used to optimize generator by maximizing $p(y | x, \mathcal{Z}_{retr} ; \rho)$, but to optimize the retriever, we need a better estimation of its probability. We thus utilize the posterior estimate conditioned on the current retrieved $\mathcal{Z}_{retr}$ and also output answer $y$:
% \begin{align}
%           & p(Z=\mathcal{Z}_{retr} \mid x, y; \theta, \rho) \\
% \propto \ & p(Z=\mathcal{Z}_{retr} \mid x; \theta) \cdot p(y \mid x, Z=\mathcal{Z}_{retr}; \rho). 
% \end{align}

% The first term could be simply modified Eq.(\ref{eq:retrieve}) by only summation over the top k knowledge in $\mathcal{Z}_{retr}$. The second term is measuring how important each knowledge $z_i$ is for the model to correctly generate the answer.


\paragraph{Online Retrieval over Asynchronous Updated Memory}
Note that in the E-Step, we need to find Top-K knowledge. With bi-encoder as retriever, we could simply use the relevance score $Rel(x,z) = \texttt{Embed}_Q(x)^T \cdot \texttt{Embed}_K(z^j_i) \cdot Gate_{\mathcal{C}^j}(x)$ to rank the ordering of knowledge. This is a standard Maximum Inner Product Search (MIPS) problem and we could use approximate algorithms~\cite{DBLP:conf/nips/Shrivastava014, DBLP:journals/corr/abs-2206-14286} that scale sub-linearly with the size of knowledge corpus $|C|$.

After identifying the Top-K knowledge $\mathcal{Z}_{retr}$ via MIPS, we need to get $K$ compressed knowledge embeddings $\psi(f(z_i)), \forall z_i \in \mathcal{Z}_{retr}$. If we want to scale the retrieved number $K$ to hundred, this re-calculation could be very time consuming. Therefore, we propose to store all the stale knowledge embeddings in a online knowledge memory. In this way, at each retrieval step, we only re-calculate the up-to-dated embedding for a small portion (i.e., 10$\%$ of knowledge) from raw data, and for remaining ones we simply reuse the pre-computed stale embeddings.
We update the key and knowledge memory embeddings asynchronously every 1000 training steps similar to~\cite{DBLP:journals/corr/abs-2002-08909}, and store both the key memory embeddings distributedly over all online devices. 






% We plan to build a multi-modal knowledge base from different sources, including unstructured wikipedia and inside images, as well as structured knowledge graph such as Wikidata and conceptnet
% The key challenge is that we don’t have direct supervision about which entries are the ground-truth knowledge to each QA pairs, and thus we need some weekly supervision to train such system.
% On the other hand, existing VQA datasets are mostly very small and insufficient to train a large model, especially with an additional retrieval module.
% Therefore, our solution to this problem is to conduct retrieval-augmented pre-training over web-scale image caption datasets.
% Internal Google, we have Web Image Text and Webli that are billion scale image-caption.
% By taking the complex captions from these datasets, for example, identifying that this image is Theodore Roosevelt at Pennsylvania, the model is guided to retrieve the relevant knowledge via end2end pre-training

\subsection{Generative Pre-Training Details of \method}
With the model architecture introduced above, \method is able to be trained end-to-end via only the generation loss. 


Note that in our downstream tasks, we'd like our model to handle different multimodal input $x$, including text-only, image-only and image-text pairs. We thus utilize the Prefix Language Modeling (PreLM) utilized in SimVLM~\cite{DBLP:conf/iclr/WangYYDT022} as main objective. Given image text pairs ($x, I)$ from pre-training dataset corpus $\mathcal{D}$.
we randomly sample a prefix length $L_{p}$, and treat prefix $x_{<L_{p}}$ (containing both image and text query) as condition to autoregressively generate remaining text sequence $x_{\geq L_{p}}$:
{\small
\begin{align}
    \mathcal{L}_{\text{PreLM}} = & -\mathbb{E}_{(x,I) \sim \mathcal{D}}  \big[ {\log p(x_{\geq L_{p}} \mid I, x_{<L_{p}}; \theta, \rho, \mathcal{C} )}  \big] \\
   = &  -\mathbb{E}_{(x,I) \sim \mathcal{D}} \Big[ \sum_{t \geq L_{p}} {\log p(x_t \mid x_{[L_{p}, t)},I, x_{<L_{p}}; \theta, \rho, \mathcal{C} )  } \Big] \nonumber  
\end{align}
}
We then could involve our knowledge retriever into the objective via Eq.(\ref{eq:main}) to jointly train retriever and generator. 


\paragraph{Model Initialization}
Similar to previous retrieval-augmented models, if at the beginning the retrieval model is not initialized properly, the retrieved knowledge $\mathcal{Z}$ are likely to be unrelated to the query $x$. In this situation, retriever does not receive meaningful gradients to update the parameters, and generator learns to ignore the knowledge.  
To avoid this cold-start problem and provide retriever a good initialization, We propose to construct pseudo ground-truth knowledge to give model a reasonable initialization. We utilize the Wikipedia-Image-Text (WIT)~\cite{DBLP:conf/sigir/Srinivasan0CBN21} dataset for such purpose. For each image-caption pair in WIT, they also provide the corresponding Wikipedia passage, and thus we treat $\hat{z}=  $($\text{wiki passage}, I$) as ground-truth knowledge pairs. As the passage provide rich information about generated caption, it definitely is useful for the task and could help initialize the model. To avoid the model simply utilize low-level image feature to find out such ground-truth result, we adopt: 1) image augmentation including random cropping and Gaussian blur; 2) randomly drop out the whole image, so the retriever needs to identify image-text correspondence. After initializing over WIT and switching to larger-scale web image-caption datasets, we no longer have access to ground-truth text passage, and thus a naive choice as ground-truth retrieved results is $\hat{z}=  $($x_{\geq L_{p}}, I$) image-text pairs. As it contains the generated answer, it definitely is useful for the task. 

With such constructed pseudo retrieval ground-truth $\hat{z}$, we firstly in-batch contrastive learning, which maximize the following contrastive loss: 
\begin{align}
    &\mathcal{L}_{contra} = - \log \text{Softmax}(\texttt{Embed}_Q(x)^T \texttt{Embed}_K(\hat{z}))
\end{align}
We also randomly replace (with $p=10\%$ the retrieved knowledge with this ground-truth knowledge to guide generator utilize retrieved knowledge instead of only using input query.






% As the retrieval module of \method requires a good initialization to get high-quality Top-K knowledge set to support end-to-end training, we firstly initialize \method over Wiki-Image-Text (WIT) dataset with pseudo supervised ground-truth. We then froze the base V-L encoder and conduct end-to-end pre-training over large-scale but more noisy web image-text dataset. We utilize English-dump of WebLI~\cite{https://doi.org/10.48550/arxiv.2209.06794}, a 3B web-image text dataset for generative pre-training.

% After pre-training, we freeze the learned knowledge memory and base VL-encoder, and only finetune the fusion and decoder part for various knowledge-intensive downstream tasks, such as VQA.























% Here let me introduce the overall architecture. We first introduce the most standard image2text workflow.
% Taking a image caption from wikipedia as an example. We first extract uni-modal image and text features with a VL encoder.
% And then, we fuse the two modality via a neural fusion layer, and pass them to decoder.
% Without outside knowledge, the model needs to generate “Zizania species” given only image as input, which is hard as the model parameter is hard to memorize so much rare entities.
% Therefore, in the forward pass, we allow the model to get access a dynamically updated knowledge memory.
% We utilize the wikipedia as knowledge corpus, each key and value in the memory represents a single image-passage pair in wikipedia pages. We update the memory asynchronous via pre-training.
% During model forward pass, we conduct on-TPU MIPS dense retrieval for approximate top-k results.
% Given the retrieved top-K knowledge, we multiple each with the retrieval score calculated within these K entries, multiply each knowledge value by the score, and pass to a knowledge fusion layer. In this way, the retrieval could be end2end updated via our caption generation task.
% Eventually, if one of the retrieved knowledge contains Zizania information, the corresponding knowledge will receive positive gradient, and the decoder could utilize better retrieved knowledge to generate hard tokens.
% After pre-training, we freeze the learned knowledge memory and base VL-encoder, and only finetune the fusion and decoder part for various knowledge-intensive downstream tasks, such as VQA.


